Unsupervised Hashing with Similarity Distribution Calibration

Unsupervised hashing methods typically aim to preserve the similarity between data points in a feature space by mapping them to binary hash codes. However, these methods often overlook the fact that the similarity between data points in the continuous feature space may not be preserved in the discrete hash code space, due to the limited similarity range of hash codes. The similarity range is bounded by the code length and can lead to a problem known as similarity collapse. That is, the positive and negative pairs of data points become less distinguishable from each other in the hash space. To alleviate this problem, in this paper a novel Similarity Distribution Calibration (SDC) method is introduced. SDC aligns the hash code similarity distribution towards a calibration distribution (e.g., beta distribution) with sufficient spread across the entire similarity range, thus alleviating the similarity collapse problem. Extensive experiments show that our SDC outperforms significantly the state-of-the-art alternatives on coarse category-level and instance-level image retrieval. Code is available at https://github.com/kamwoh/sdc.

==> tables/algorithm.tex <==
% \begin{algorithm}[t]
% \caption{\shortname{} Loss Function.}
% \label{alg:sdp}
% \definecolor{codeblue}{rgb}{0.25,0.5,0.5}
% \lstset{
%   backgroundcolor=\color{white},
%   basicstyle=\fontsize{7.2pt}{7.2pt}\ttfamily\selectfont,
%   columns=fullflexible,
%   breaklines=true,
%   captionpos=b,
%   commentstyle=\fontsize{7.2pt}{7.2pt}\color{Gray},
%   keywordstyle=\fontsize{7.2pt}{7.2pt},
% %  frame=tb,
% }
% \begin{lstlisting}[language=python]
% # phi: non-linear hash layer
% # N: number of pairs (half of the batch)
% # x: features (2N, d)

% # compute continuous codes    
% f = <@\textcolor{Purple}{\textbf{phi}}@>(x) # (2N, k)

% # construct pairs
% xi, xj = x[:N], x[N:]  # (N, d)
% fi, fj = f[:N], f[N:]  # (N, k)
% t, t_idx = <@\textcolor{Purple}{\textbf{sort}}@>(<@\textcolor{Purple}{\textbf{cossim}}@>(xi, xj)) # (N,)
% s = <@\textcolor{Purple}{\textbf{cossim}}@>(fi, fj) # (N,)

% # sort with t's index
% s = s[t_idx] # (N,)

% # inverse CDF of beta distribution
% C = <@\textcolor{Purple}{\textbf{beta
% \_ppf}}@>(N, alpha=5, beta=5).<@\textcolor{Purple}{\textbf{relu}}@>() # (N,)

% loss_sdc = (s - C).<@\textcolor{Purple}{\textbf{abs}}@>().<@\textcolor{Purple}{\textbf{mean}}@>()
% loss_q = (1 - <@\textcolor{Purple}{\textbf{cossim}}@>(f, f.<@\textcolor{Purple}{\textbf{sign}}@>())).<@\textcolor{Purple}{\textbf{mean}}@>()
% loss = loss_sdc + lambda_q * loss_q
    
% \end{lstlisting}
% \end{algorithm}



\begin{algorithm}[t]
\caption{\shortname{} Loss Function.}
\label{alg:sdp}
\definecolor{codeblue}{rgb}{0.25,0.5,0.5}
\lstset{
  backgroundcolor=\color{white},
  basicstyle=\fontsize{7.2pt}{7.2pt}\ttfamily\selectfont,
  columns=fullflexible,
  breaklines=true,
  captionpos=b,
  commentstyle=\fontsize{7.2pt}{7.2pt}\color{gray},
  keywordstyle=\fontsize{7.2pt}{7.2pt},
%  frame=tb,
}
\begin{lstlisting}[language=python]
# phi: non-linear hash layer
# N: number of pairs (half of the batch)
# x: features (2N, d), x2: features of randomly augmented input (2N, d)

# compute continuous codes    
f = <@\textcolor{violet}{\textbf{phi}}@>(x) # (2N, k)

# construct pairs
xi, xj = x[:N], x[N:]  # (N, d)
fi, fj = f[:N], f[N:]  # (N, k)
t, t_idx = <@\textcolor{violet}{\textbf{sort}}@>(<@\textcolor{violet}{\textbf{cossim}}@>(xi, xj)) # (N,)
s = <@\textcolor{violet}{\textbf{cossim}}@>(fi, fj) # (N,)

# sort with t's index
s = s[t_idx] # (N,)

# inverse CDF of beta distribution
C = <@\textcolor{violet}{\textbf{beta
\_ppf}}@>(N, alpha=5, beta=5) # (N,)

# contrastive loss with simclr
loss_cl = <@\textcolor{violet}{\textbf{SimCLR}}@>(x, x2)

loss_sdc = (s - C).<@\textcolor{violet}{\textbf{abs}}@>().<@\textcolor{violet}{\textbf{mean}}@>()
loss_q = (1 - <@\textcolor{violet}{\textbf{cossim}}@>(f, f.<@\textcolor{violet}{\textbf{sign}}@>())).<@\textcolor{violet}{\textbf{mean}}@>()
loss = loss_sdc + lambda_q * loss_q + lambda_cl * loss_cl
    
\end{lstlisting}
\end{algorithm}

==> tables/fig_disthist_orig_and_ugh.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.3, keepaspectratio=True]{figures/disthistogram_cifar10orig_4096.pdf}
    \includegraphics[scale=0.3, keepaspectratio=True]{figures/disthistogram_cifar10_ugh_64_no_yaxis.pdf}
    \caption{Pairwise similarity distribution of CIFAR10 using 100k randomly chosen negative pairs and 10k positive pairs. \textbf{(Left)} VGG16 features. \textbf{(Right)} 64-bits hash codes of GreedyHash \cite{greedyhash2018su}. Note that, the positive and negative labels are included for ease of explanation (\ie descriptive purpose only), and were not deployed during the actual unsupervised training.}
    \label{fig:disthist_orig_and_ugh}
\end{figure}

==> tables/fig_teaser.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[keepaspectratio=True, scale=0.35]{figures/aaai2023diagram-verticalv2.pdf}
    \caption{
    \textbf{(a)} Original continuous features (before hashing) and the cosine similarity distribution 
    of positive (green) and negative (red) pairs.
    \textbf{(b)} 
    After mapping to the hash code space under feature similarity preservation,
    the similarity collapse phenomenon happens due to the limited similarity capacity in Hamming space and the original similarity bias. 
    \textbf{(c)} This problem can be well alleviated 
    by our {\em \modelname{}} method. 
    } 
    \label{fig:bigteaser}
    % \vspace{-0.3cm}
\end{figure}

==> tables/tab_architecture_performance.tex <==
\begin{table*}[t]
    \centering
    \begin{adjustbox}{max width=0.95\textwidth}
        \begin{tabular}{l|cccc|cccc}
        \hline
        \multirow{2}{*}{Methods} & \multicolumn{4}{c|}{ResNet50 \cite{resnet2015he}} & \multicolumn{4}{c}{DeiT-S \cite{deit2021touvron}} \\
        \cline{2-9}
        & CIFAR10 & ImageNet100 & NUSWIDE & MS-COCO & CIFAR10 & ImageNet100 & NUSWIDE & MS-COCO \\
        \hline
        ITQ \cite{itq2012gong} & 64.6 & 73.9 & 79.5 & 75.3 & 80.4 & 74.7 & 79.2 & 78.4 \\
        GreedyHash \cite{greedyhash2018su} & 61.4 & 77.9 & 83.0 & 77.6 & 81.5 & 79.7 & 80.8 & 80.8 \\
        BiHalf \cite{bihalf2021li} & 76.6 & 80.4 & 82.7 & 78.5 & 79.9 & \textbf{81.3} & 74.5 & 79.7 \\
        % \textbf{SDP (Ours)} & \textbf{77.7} & \textbf{89.3} & \textbf{83.3} & \textbf{82.5} & \textbf{88.7} & \textbf{86.2} & \textbf{83.4} & \textbf{84.9} \\
        % \bf SDP (Ours) & \textbf{78.5} & \textbf{84.9} & 82.9 & \textbf{80.1} & \textbf{90.0} & \textbf{81.3} & \textbf{82.8} & \textbf{82.8} \\
        \bf \shortname{} (Ours) & \bf 78.7 & \bf 85.1 & \bf 83.7 & \bf 81.3 & \bf 89.5 &  80.7 & \bf 83.3 & \bf 82.9 \\
        \hline
        \textit{Original Features} & 69.3 & 81.8 & 83.9 & 82.1 & 82.3 & 82.5 & 83.9 & 84.2 \\
        \hline
        \end{tabular}
    \end{adjustbox}
    \caption{Coarse category-level image retrieval results of representative unsupervised hashing methods on ImageNet100. 64-bits hash codes are used.
    The last row reports the results of the original 2048d ResNet50 and 384d DeiT-S features.
    }
    \label{tab:architecture_performance}
    % \vspace{-0.1cm}
\end{table*}

==> tables/tab_beta.tex <==
% \begin{table}[t]
%     \centering
%     \begin{adjustbox}{max width=0.95\linewidth}
%         \begin{tabular}{c|ccc}
%         \hline
%             Distributions & CIFAR10 & ImageNet100 & GLDv2 \\
%             \hline
%             \texttt{Beta}$(0.2, 0.2)$ & 62.2 & 79.7 & 11.6 \\
%             \texttt{Beta}$(0.5, 0.5)$ & 63.6 & 80.6 & 11.9 \\
%             \texttt{Beta}$(0.7, 0.7)$ & 64.1 & 80.8 & 11.8 \\
%             \texttt{Beta}$(1, 1)$ & 66.2 & 80.8 & 12.0 \\
%             \texttt{Beta}$(2, 2)$ & 67.0 & 81.4 & \bf 12.1 \\
%             \texttt{Beta}$(3, 3)$ & \bf 67.3 & 81.9 & 12.0 \\
%             \texttt{Beta}$(5, 5)$ & \bf 67.3 & 82.9 & \bf 12.1 \\
%             \texttt{Beta}$(7, 7)$ & 66.8 & 82.8 & 11.8 \\
%             \texttt{Beta}$(10, 10)$ & 65.9 & \bf 83.3 & 11.8 \\
%             \hline
%             \texttt{Gaussian} & \textbf{67.3} & 82.3 & 11.5 \\
%             \hline
%         \end{tabular}
%     \end{adjustbox}
%     \caption{
%     Effect of the calibration distribution.
%     % Performance of using different hyperparameters of $\alpha$ and Gaussian distribution. 
%     {\em Setting}: 64-bits hash codes on CIFAR10 and ImageNet and 512-bits on GLDv2.}
%     \label{tab:beta}
%     % \vspace{-0.1cm}
% \end{table}

% 59.8 64.0 66.3 72.8 78.5 80.6

\begin{table}[t]
    \centering
    \begin{adjustbox}{max width=0.95\linewidth}
        \begin{tabular}{c|ccc}
        \hline
            Distributions & CIFAR10 & ImageNet100 & GLDv2 \\
            \hline
            \texttt{Beta}$(0.2, 0.2)$ & 19.3 & 70.3 & 11.6 \\
            \texttt{Beta}$(0.5, 0.5)$ & 54.8 & 76.3 & 11.9 \\
            \texttt{Beta}$(0.7, 0.7)$ & 55.9 & 77.2 & 11.8 \\
            \texttt{Beta}$(1, 1)$ & 58.4 & 79.0 & 12.0 \\
            \texttt{Beta}$(2, 2)$ & 62.5 & 80.5 & \bf 12.1 \\
            \texttt{Beta}$(3, 3)$ & 62.5 & 80.6 & 12.0 \\
            \texttt{Beta}$(5, 5)$ & \bf 63.0 & 80.6 & \bf 12.1 \\
            \texttt{Beta}$(7, 7)$ & 62.6 & \bf 82.2 & 11.8 \\
            \texttt{Beta}$(10, 10)$ & 61.3 & 81.7 & 11.8 \\
            \hline
            \texttt{Gaussian} & 62.6 & 80.5 & 11.5 \\
            \hline
        \end{tabular}
    \end{adjustbox}
    \caption{
    Effect of the calibration distribution.
    % Performance of using different hyperparameters of $\alpha$ and Gaussian distribution. 
    {\em Setting}: 64-bits hash codes on CIFAR10 and ImageNet and 512-bits on GLDv2.}
    \label{tab:beta}
    % \vspace{-0.1cm}
\end{table}

% 59.8 64.0 66.3 72.8 78.5 80.6

==> tables/tab_cs_before_and_after.tex <==
\begin{table}[t!]
    \centering
    \caption{Effect of whitening on the cosine similarity
        in terms of the average and the entropy.
        Original features: VGG-16.}
    %\vspace{-1em}
    \label{tab:cs_before_and_after}
    \begin{adjustbox}{max width=\textwidth}
        \begin{tabular}{l|c|c}
        \hline
        Datasets & Average
        %$\mathbb{E}[\mathcal{D}]$
        & Entropy %$H(\mathbf{T})$
        \\
        \hline
        CIFAR10 & 0.4775$\xrightarrow{}$\textbf{0.3701} & 2.4774$\xrightarrow{}$\textbf{2.6350} \\
        ImageNet100 & 0.1176$\xrightarrow{}$\textbf{0.0068} & 1.9633$\xrightarrow{}$\textbf{2.0270} \\
        NUS-WIDE & 0.2233$\xrightarrow{}$\textbf{0.0996} & 2.6550$\xrightarrow{}$\textbf{2.7209} \\
        MS-COCO & 0.1497$\xrightarrow{}$\textbf{0.0312} & 2.2483$\xrightarrow{}$\textbf{2.3045} \\
        \hline
        \end{tabular}
    \end{adjustbox}
\end{table}


==> tables/tab_instance_performance.tex <==
\begin{table}[t]
    %\vspace{-1em}
    \centering
    \begin{adjustbox}{max width=0.95\linewidth}
        \begin{tabular}{l|cc|cc|cc}
        \hline
        \multirow{2}{*}{Methods} & \multicolumn{2}{c|}{GLDv2} & \multicolumn{2}{c|}{$\mathcal{R}$Oxf} & \multicolumn{2}{c}{$\mathcal{R}$Paris} \\
        \cline{2-7}
        & 128 & 512 & 128 & 512 & 128 & 512 \\
        \hline
        ITQ \cite{itq2012gong} & 5.2 & 11.3 & 1.6 & 5.4 & 4.8 & 12.3 \\
        % \hline
        GreedyHash \cite{greedyhash2018su} & 3.8 & 7.9 & 15.8 & 34.2 & 34.9 & 52.8 \\
        BiHalf \cite{bihalf2021li} & 4.0 & 6.7 & 20.2 & 33.3 & 42.0 & 52.0 \\
        \bf \shortname{} (Ours) & \textbf{6.3} & \textbf{12.1} & \textbf{27.1} & \textbf{40.8} & \textbf{50.3} & \textbf{63.8} \\
        \hline
        \em Original features
        & \multicolumn{2}{c|}{13.8} & \multicolumn{2}{c|}{51.0} & \multicolumn{2}{c}{71.5} \\
        \hline
        \end{tabular}
    \end{adjustbox}
    \caption{Instance-level image retrieval results of representative unsupervised hashing methods on GLDv2, $\mathcal{R}$Oxf-\textbf{Hard} and $\mathcal{R}$Paris-\textbf{Hard}. 
    % R50-DELG-C:
    Original features: 2048D R50-DELG features \cite{delg2020cao} with the cosine similarity.
    % cosine distance retrieval using the extracted descriptors (2048-d vector).
    }
    \label{tab:instance_performance}
    % \vspace{-0.2cm}
\end{table}

==> tables/tab_loss.tex <==

\begin{table}[t]
    \centering
    \begin{adjustbox}{max width=0.95\linewidth}
        \begin{tabular}{c|ccc}
        \hline
            Orthogonality Constraint & CIFAR10 & ImageNet100 & GLDv2 \\
             \hline
             % $(\hat{t}_n^\dagger - F^{-1}(\frac{2n-1}{2N}))^2$ & 66.9 & 81.7 & 8.4 \\
             \Tstrut
            No & 64.9 & 81.1 & 7.2 \\
            \Tstrut
            Yes & \textbf{67.3} &\bf 82.9 & \textbf{12.1} \\
            \hline
        \end{tabular}
    \end{adjustbox}
    \caption{Effect of orthogonality.
    {\em Setting}: 64-bits hash codes on CIFAR10 and ImageNet and 512-bits on GLDv2.
    % 64-bits hash codes are used on CIFAR10 and ImageNet and 512-bits hash codes are used on GLDv2.
    }
    % \vspace{-0.2cm}
    \label{tab:simloss}
\end{table}
